Poset vectors and generalized permutohedra

We show that given a poset P and and a subposet Q, the integer points obtained by restricting linear extensions of P to Q can be explained via integer lattice points of a generalized permutohedron.

==> header.tex <==
\pagestart{1}

\pageend{12}
\authorhead{Dorian Croitoru and Suho Oh and Alexander Postnikov}
\titlehead{Poset vectors and generalized permutohedra}
\titlelong{Poset vectors and generalized permutohedra (extended abstract)}
\keywords{Poset, linear extension, associahedron, generalized permutohedra, polytope, integer lattice points}


